Improved algorithms for online load balancing

We consider an online load balancing problem and its extensions in the framework of repeated games. On each round, the player chooses a distribution (task allocation) over $K$ servers, and then the environment reveals the load of each server, which determines the computation time of each server for processing the task assigned. After all rounds, the cost of the player is measured by some norm of the cumulative computation-time vector. The cost is the makespan if the norm is $L_\infty$-norm. The goal is to minimize the regret, i.e., minimizing the player's cost relative to the cost of the best fixed distribution in hindsight. We propose algorithms for general norms and prove their regret bounds. In particular, for $L_\infty$-norm, our regret bound matches the best known bound and the proposed algorithm runs in polynomial time per trial involving linear programming and second order programming, whereas no polynomial time algorithm was previously known to achieve the bound.

==> extension.tex <==
\section{extension}
Of course we can extend the online load balancing problem i.e,. make-span from $\infty$-norm to $p$-norm, where $p>2$. By involving $p$-norm algorithm \cite{shalev2012online} we may extend our algorithm to $p$-norm. First we state this problem in following.

For $p >2,$ consider the global cost function $C(x)=\Vert x\Vert_{p}$ and $C^{*}(x)=\min_{\alpha \in \Delta{K}}\Vert \alpha \odot x\Vert_{p}.$ So our regret is as follow:
$$\mathrm{Reg}_{T}=C(L_{T}^{A})-C^{*}(L_{T}).$$

Now we give the target set
$$S=\lbrace (x,y) \in \mathbb{R}^{k} \times \mathbb{R}^{k}: x_{i}, y_{i} \in  [0,1]; C(x) \leq C^{\star}(y) \rbrace.$$

\begin{algorithm}
\caption{An algorithm for p-norm}
\label{alg:An-algorithm-for-p-norm}
\begin{algorithmic}
\REQUIRE First we give the target set $S$ as above, and
$w_{0}=0,$ $\theta_{0}=0$ and $\alpha_{0}=(1/K, \cdots, 1/K).$ We let $r_{t}=(\alpha_{t} \odot \l_{t},l_{t}).$
\FOR {$t=1, \cdots, T$}
\STATE 1. We calculate that $s_{0}^{*}=\mathrm{SOCP}(w_{0}).$

\STATE 2. At round $t=1, \cdots, T,$ choose $\alpha_{t}$ such that
\begin{equation}
\alpha_{t}=\argmin_{\alpha}\max_{l \in [0,1]^{K}}\langle w_{t}, (\alpha \odot l,l)\rangle,
\end{equation}
where we update $w_{t}(i)=\eta\frac{\sgn(\theta_{t}(i))|\theta_{t}(i)|^{p-1}}{\Vert \theta_{t}\Vert_{p}^{p-2}},$ and
$\theta_{t}=\theta_{t-1}-(-r_{t}+s_{t}^{*}),$
where $s_{t}^{*}=\mathrm{SOCP}(w_{t}).$
\ENDFOR
\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{theorem:p-norm}
For online global cost function, if we run the above algorithm $T$ times. Then we may give the upper bound to regret of online learning with global cost function in following:
\begin{equation}
C(L_{T}^{A})-C^{*}(L_{T}) \leq 2^{(p-1)/p}K^{1/p}\sqrt{\frac{2p}{T}}
\end{equation}
\end{theorem}

We give the proof of our theorem in appendix.




==> proof.tex <==
\section{Proof}
In this section we give the proof of the Theorem \ref{regret:make-span}. Briefly speaking the proof of this theorem is consisted in two parts. In the first part we give a reduction from the regret of load balancing problem to Blackwell approachability. In this part we state that regret of load balancing can be bounded by the $L_{\infty}$-norm distance from the average payoff vector to $S.$ In the second part, \cite{shimkin2016online} proves that this distance can be bounded by regret of Online Convex Optimization(OCO) originally. However in our paper we give another idea of proof, which is directly from Linear Programming in our algorithm.
\begin{proof}(Theorem \ref{regret:make-span})
Since we have proven that $S$ is approachable, we know that the existence of $\alpha_{t}$ is guaranteed. In the following part we are going to prove the upper bound of the regret. By the approachability of our target set we can find a point $(x,y) \in S$ such that $s=(x,y)=\argmin_{s \in S}\Vert \bar{r}_{T}-s\Vert_{\infty}.$ Hence we have that
\begin{equation*}
\begin{split}
C(L_{T}^{A})-C^{\star}(L_{T}) &=[C(x)-C^{\star}(y)]+[C(L_{T}^{A})-C(x)]+[C^{\star}(y)-C^{\star}(L_{T})] \\
& \leq 1 (\Vert L_{T}^{A}-x \Vert_{\infty}+ \Vert L_{T}-y \Vert_{\infty}) \\
& \leq 1 \Vert 2((L_{T}^{A}, L_{T})-(x,y)) \Vert_{\infty} \\
& = 2\Vert \bar{r}_{T}-(x,y) \Vert_{\infty}, \\
\end{split}
\end{equation*}
where the first inequality is from the definition of $S.$

By lemma \ref{lemma:distance} we know that
\begin{equation*}
\begin{split}
\Vert \bar{r}_{T}-(x,y) \Vert_{\infty}&= \max_{\Vert w \Vert_{1} \leq 1} \left(\langle \bar{r}_{T}, w\rangle -h_{S}(w)\right) \\
&=-\min_{\Vert w \Vert_{1} \leq 1}\left( \langle -\bar{r}_{T}, w\rangle +h_{S}(w)\right).
\end{split}
\end{equation*}

In the following part we denote that $w_{*}=w^{+}_{*}-w^{-}_{*}=\argmin_{\Vert w \Vert_{1} \leq 1}\left(\langle -\bar{r}_{T},w \rangle +h_{S}(w)\right),$ and for this $w_{*}$ there is $s_{*} \in S$ such that $s_{*}=\argmax_{s \in S} \langle s, w_{*}\rangle.$

Now by involving the KL-divergence we have that
\begin{equation*}
\begin{split}
&\mathrm{KL}(w_{*}^{+}\Vert w_{t}^{+})-\mathrm{KL}(w_{*}^{+}\Vert w_{t+1}^{+})=\sum_{i=1}^{2d} w_{*}^{+}(i) \ln \frac{w_{t+1}^{+}(i)}{w_{t}^{+}(i)} \\
&= \sum_{i=1}^{2d} w_{*}^{+}(i) \cdot \left(-\eta (-r_{t}+s_{t}^{*})-\ln \left(\sum_{j=1}^{2d} w_{t}^{+}(j)e^{-\eta (-r_{t}+s_{t}^{*})}+w_{t}^{-}(j)e^{\eta (-r_{t}+s_{t}^{*})}\right)\right)
\end{split}
\end{equation*}

From above equations we may have
\begin{equation*}
\begin{split}
&\sum_{t=1}^{T}(\mathrm{KL}(w_{*}^{+}\Vert w_{t}^{+})-\mathrm{KL}(w^{+}_{*}\Vert w_{t+1}^{+}))+(\mathrm{KL}(w_{*}^{-}\Vert w_{t}^{-})-\mathrm{KL}(w^{-}_{*}\Vert w_{t+1}^{-})) \\
&\geq -2\sum_{t=1}^{T} \ln \left(\sum_{j=1}^{2d} w_{t}^{+}(j)e^{-\eta (-r_{t}+s_{t}^{*})}+w_{t}^{-}(j)e^{\eta (-r_{t}+s_{t}^{*})}\right) \\
& + \sum_{t=1}^{T} (w_{*}^{+}-w_{*}^{-}) \cdot [-\eta (-r_{t}+s_{t}^{*})], \\
\end{split}
\end{equation*}
since KL-divergence is always non-negative.

This is equivalent to
\begin{equation*}
\begin{split}
&\mathrm{KL}(w_{*}^{+}\Vert w_{1}^{+})+ \mathrm{KL}(w_{*}^{-}\Vert w_{1}^{-}) + 2\sum_{t=1}^{T} \ln \left(\sum_{j=1}^{2d} w_{t}^{+}(j)e^{-\eta (-r_{t}+s_{t}^{*})}+w_{t}^{-}(j)e^{\eta (-r_{t}+s_{t}^{*})}\right) \\
& \geq T (w^{+}_{*}-w^{-}_{*}) \cdot \left[ -\eta\left(\frac{\sum_{t=1}^{T}-r_{t}}{T}\right)+\frac{\sum_{t=1}^{T}s_{t}^{*}}{T} \right] \\
& \geq -T\eta \min_{\Vert w\Vert_{1} \leq 1}[-\langle \bar{r}_{T},w\rangle +h_{S}(w)] \\
\end{split}
\end{equation*}

By H$\mathrm{\ddot{o}}$ffding's inequality \cite{hoeven2018many}(Appendix B) we have that
\begin{equation*}
\begin{split}
&\sum_{t=1}^{T} \ln \left(\sum_{j=1}^{2d} w_{t}^{+}(j)e^{-\eta (-r_{t}+s_{t}^{*})}+w_{t}^{-}(j)e^{\eta (-r_{t}+s_{t}^{*})}\right) + \sum_{t=1}^{T} \langle w_{t}^{+}-w_{t}^{-}, -r_{t}+s_{t}^{*} \rangle \\
&\leq \frac{T\eta^{2}}{2}
\end{split}
\end{equation*}

Since the choice of the algorithm we know that the second term from the left hand side is always positive. Combining the above we have that
\begin{equation}
\mathrm{KL}(w_{*}^{+}\Vert w_{1}^{+})+ \mathrm{KL}(w_{*}^{-}\Vert w_{1}^{-}) +2 \cdot\frac{T\eta^{2}}{2} \geq -T\eta \min_{\Vert w\Vert_{1} \leq 1}[-\langle \bar{r}_{T},w\rangle +h_{S}(w)]
\end{equation}

This equation leads that:
\begin{equation*}
 -T\eta \min_{\Vert w\Vert_{1} \leq 1}[-\langle \bar{r}_{T},w\rangle +h_{S}(w)] \leq  2 \ln(4K)+ \frac{2T\eta^{2}}{2}
\end{equation*}

By choosing $\eta=\sqrt{\frac{2\ln 4K}{T}}$ then we can have
\begin{equation*}
C(L_{T}^{A})-C^{\star}(L_{T}) \leq 2\sqrt{\frac{2\ln 4K}{T}}.
\end{equation*}

\end{proof}

